From the Greene--Wu Convolution to Gradient Estimation over Riemannian Manifolds

Over a complete Riemannian manifold of finite dimension, Greene and Wu introduced a convolution, known as Greene-Wu (GW) convolution. In this paper, we study properties of the GW convolution and apply it to non-Euclidean machine learning problems. In particular, we derive a new formula for how the curvature of the space would affect the curvature of the function through the GW convolution. Also, following the study of the GW convolution, a new method for gradient estimation over Riemannian manifolds is introduced.

==> tex/algo.tex <==


\section{Gradient Estimation}

% The domain $\D$ is geodesically convex and compact. 

In each iteration, we can only pick a point to query the function value. With this information only, we need to perform a gradient step so that we find the minimum. In order to do this, we perform the the following three steps in each iteration. First, we approximate the gradient with a single-point estimate (Line 5-6 in Algorithm \ref{alg}). Second, we perform a gradient update with the estimated gradient (Line 7 in Algorithm \ref{alg}). 
Third we project the point back to a subset of the domain (Line 8 in Algorithm \ref{alg}). After the three steps, the next iteration start. 

In the first step, the gradient at $p$ is estimated by
\begin{align}
     \nabla f\big|_p \approx  \frac{n}{\delta} f \( \Exp_p (\delta v) \) v , \quad \text{with }  v \sim \S_p. 
\end{align}
% missing citation 
This estimation generalizes that by \citet{flaxman2005online} and is easy to implement. In particular, we only need to sample a tangent vector $v \in T_p \M$, compute an exponential map and observe function value at $f \( \Exp_p (\delta v) \)$. This implementation advantage is due to the algorithm design by avoiding explicitly invoking the Stokes' theorem, as we will discuss in the next section. 

The second step is to carry out a standard gradient update via exponential map. More specifically, if we are at $x_t$ and $ w_t $ is the gradient estimate for iteration $t$, the gradient update moves us to $ \Exp_{x_t } (-\eta w_t) $ where $\eta$ is the step size or learning rate. 


In the third step, we need to project the point back to a subset of the domain, which we now define. For the compact and geodesically convex domain $\D$, define 
% For a geodesically convex set compact $\D \subseteq \M$ and $\alpha > 0$, we use $ (1 - \alpha) \D $ to denote the set such that 
\begin{align}
    &(1 - \alpha ) \D := \Bigg\{ p \in \D: 
    \Exp_p (\alpha v) \in \D, \, \forall v \in \S_p \Bigg\}. \nonumber
\end{align}

% This set $(1 - \alpha) \D$ is also convex. 
We have the following proposition for this set $(1 - \alpha) \D$. 

\begin{proposition}
    The set $ (1 - \alpha ) \D $ is geodesically convex. 
\end{proposition}

\begin{proof}
    For any points $ p, q \in (1 - \alpha ) \D $, let $\gamma: [0,1] \rightarrow \M$ be the geodesic connecting $p$ to $q$, with $\gamma(0) = p$ and $\gamma (1) = q$. 
    We will show that this curve $\gamma$ is contained in $(1 - \alpha ) \D$. 
    % Let $r $ be a point on $\gamma$ such that $d(r,p) = \epsilon$. 
    Let $r_0 = p, r_2, \cdots, r_m = 1$ be points on $\gamma$ so that $ d (r_{k-1}, r_k) = \frac{d(p,q)}{m} $. 
    
    Suppose, in order to get a contradiction, that $r_1 \notin (1 - \alpha) \D$. By definition of $ (1 - \alpha) \D $, there exists $s $ such that $ d ( s , r_1 ) \le \alpha $ and $ s \notin (1 - \alpha) \D$. 
    Thus there exists a number $\epsilon_0 > 0$ such that $d (p , s ) \ge \alpha + \epsilon_0$. Otherwise, $p$ will not be in $(1 - \alpha) \D$. 
    By triangle inequality, $d (p, r_1) \ge d ( s, p ) - d ( s, r_1 )  \ge \epsilon_0$. 
    % Since the geodesic $\gamma$ is smooth. 
    Since $d(p,q)$ is fixed, we can pick a large enough $ m $, so that $ d (p, r_1) < \epsilon_0 $, which leads to a contradiction. 
    
    Inductively, this means all $r_1, r_2, \cdots, r_m \in (1 - \alpha) \D$. 
    
    Now, we can repeat the above argument and get: $ r (t) \in (1 - \alpha) \D $ for all $ t \in [0,1] \cap \mathbb{Q} $. Since $\gamma$ is a smooth curve, we have $\gamma$ is contain in $(1 - \alpha) \D$ entirely. 
\end{proof}

Since $(1 - \alpha ) \D$ is convex in a Hadamard space, the projection onto $(1 - \alpha) \D$ is properly defined. We use $ \Proj_{(1 - \alpha ) \D} (p) $ to denote projection of $p$ onto $(1 - \alpha ) \D$, which gives the point in $ (1 - \alpha ) \D $ with the smallest distance to $p$. 

Now we formally summarize our strategy in Algorithm \ref{alg}. 

% \begin{align}
%     d
% \end{align}
% if we use a generalized Stokes' theorem or divergence theorem, the computation would involve high order differential forms, or parallel transport of . Instead, 

\begin{algorithm}[t]
    \caption{}  
    \label{alg}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        \STATE \textbf{Input:} Algorithm parameter: $\delta$; $\eta$; time horizon: $T$;
        % % Parameters: a truncation constant $ D $. 
        \STATE \textbf{Initialize up:} Arbitrarily pick $x_0 \in \M$. Set $\bar{x}_0 = x_0$. Observe $f(x_0)$. 
        \FOR {$t = 0, 1, 2,  \dots T-1$} 
            \STATE /* Pick a conanical basis with resepect to $g_{x_t}$ (the inner product at $x_t$). */ 
        	\STATE Sample $v_t \sim \S_{x_t} $. \STATE Observe function value at $ z_t = \Exp_{x_t} (\delta v_t ) $, and compute $ w_t = \frac{n}{\delta} f (z_t) v_t $. /* $w_t$ is the gradient estimate. */
        	\STATE Perform gradient update 
        	$x_{t+\frac{1}{2}} = \Exp_{x_t} ( -\eta w_t )$. 
        	\STATE Project the point set $(1 - \delta) \D$, $x_{t+1} = \Proj_{(1 - \delta) \D} \(x_{t + \frac{1}{2}} \) $. 
        	
        	/* In practice, the projection can be approximated by a point in $(1 - \delta) \D$ that is close to $x_{t+\frac{1}{2}}$. */
        	\STATE Compute
        	\begin{align}
        	    \bar{x}_{t+1} = \Exp_{x_t} \( \frac{1}{t+1} \Exp_{\bar{x}_t }^{-1} \( x_{t+1} \) \) . \label{eq:def-x-avg}
        	\end{align}
        % 		\begin{align} 
        % 			J_t \in \arg\max_{ v \in V } \wt{Z}_{ v, {N}_t^+  (v)  }, \nonumber
        % 		\end{align} 
        % 		where $ $ with ties broken arbitrarily. 
        % 	\STATE Observe the trajectory $ \P_{t, v_t} := \big\{ X_{t,0}, L_{t,1}, X_{t,1}, L_{t,2}, X_{t,2}, \cdots, L_{t,H_{t,v_t}} X_{t,H_{t,v_t}} \big\} $. Update ${N}_t^+ (v)$ and estimates $ \wt{Z}_{t, N_t (v)} $ for all $v \in [K]$. 
        \ENDFOR 
        \STATE \textbf{Ourput:} $\bar{x}_{T}$. 
    \end{algorithmic} 
\end{algorithm} 

% In particular, Algorithm \ref{alg} achieves $\wt{ \mathcal{O} } \(  \)$ convergence rate, as stated in Theorem \ref{thm:rate}. 

\begin{theorem}
    \label{thm:rate}
    % Let $D$ bound the diameter of domain $\D \subseteq \M$. Let $ G = \sup_{p \in \D} f (p)$. 
    Let assumptions in (\textbf{A0}) and  (\textbf{A1}) be satisfied. Let $ G = \sup_{p \in \D} f (p)$. 
    Then Algorithm \ref{alg} satisfies
    \begin{align}
        &\E_{v_1, v_2, \cdots, v_T} \[ f (\bar{x}_T) - f (x^*) \] 
        \le
        % \frac{D^2}{2\eta ,} + L \delta T + \frac{\zeta (\kappa, D) \eta n^2 G^2 }{2\delta^2 } , 
        \frac{D^2}{2\eta T } + \frac{\zeta (\kappa, D) \eta n^2 G^2 }{2\delta^2 }  + \( L + \frac{D\mu n}{2} \) \delta, \nonumber
    \end{align}
     where $ \zeta (\kappa, D) = \frac{ \sqrt{|\kappa|} D }{ \tanh (\sqrt{|\kappa|} D ) }$. 
    % In particular, with $\delta = T$ and $\eta = T$
\end{theorem}
In particular, when $ \eta = \Theta \( T^{-3/4 } \) $ and $\delta = \Theta \(  T^{-1/4} \)$, the algorithm achieves rate of order $ \mathcal{O} \( T^{-1/4} \) $. 
We will prove Theorem \ref{thm:rate} in the next section. 

\section{Analysis}
% The analysis can be decompose into three parts. 1. single point gradient estimate; 2. study of the surrogate function 3. Gradient descent analysis on the surrogate function.  

Before proceeding, we first state the following two propositions, which identify a tangent space $T_p \M$ with the Euclidean space (of the same dimension). 

% \textbf{Auxilliary Propositions:}

% \subsection{Auxiliary Propositions}

\begin{proposition} 
    \label{prop:inner-prod}
    Let $\S_p$ be the unit sphere in $T_p \M$. For any vector $u \in T_p \M $, we have 
    \begin{align} 
         \E_{ v \sim \S_p } \[ \< u, v \>_p v \] = \frac{ 1 }{ n } u . 
    \end{align} 
\end{proposition} 

\begin{proof}
    By linearity, it is sufficient to consider $u = e_i$, where $ \{ e_i \}_i$ is the local canonical basis for $T_p \M$ with respect to $g_p$.
    In particular, we can choose $\{ e_i \}_i$ such that $\< e_i, e_j \>_p = \delta_{ij}$, where $ \delta_{ij} $ is the Kronecker delta. 
%    In this case, the computation is the same as the standard Euclidean case. 
    For any $i,j \in \{1,2,\cdots, n \}$, 
    \begin{align} 
         \( \E_{ v \sim \S_p } \[ \< e_i, v \> v \] \)_j = \E_{ v \sim \S_p } \[ v_i v_j \].  
    \end{align} 
    Since $ \E_{ v \sim \S_p } \[ v_j | v_i = x \] = 0$ for any $x$ when $ i \neq j$, we have $\E_{ v \sim \S_p } \[ v_i  v_j \] = 0$. When $ i = j $, by symmetry, we have $\E_{ v \sim \S_p } \[ v_j^2 \] = \frac{1}{n}$ for all $j = 1,2,\cdots, n$. 
\end{proof} 

Also, since for any $p \in \M$, $ T_p \M $ can be isometrically identified with $\R^n$, we have the following proposition. 
\begin{proposition} 
    Let $\S_p$ be the unit sphere in $T_p \M$. It holds that the surface area of $\S_p $ is the same as the surface are of the unit ball in $\R^n$. 
\end{proposition} 

For the rest of the paper, we use $A_n := \frac{\pi^{n/2}}{ \Gamma \( \frac{n}{2} + 1\) }$ to denote the surface area of $(n-1)$-unit spheres, where $\Gamma$ is the Gamma function. 

% \begin{proof} 
    
% \end{proof} 

Next, we introduce a local surrogate function and a global convolution, which will be needed for our gradient estimation. 

\subsection{A Local Surrogate Function and a Global Convolution}

\textbf{A Local Surrogate Function} 



For a $p \in \M$ and $ v \in T_p \M $, we define
$ \wt{f}_{p,v}^\delta (q) $ in a neighborhood of $p$ so that 
\begin{align}
    \wt{f}_{p,v}^\delta(q)= \frac{1}{2\delta}\int_{-\delta}^\delta f(\Exp_q(tv_q))dt, \label{eq:fvd}
\end{align}
where $v_q := P_{0,1}^\gamma (v)$, $\gamma:[0,1]\rightarrow \M$ is the unique geodesic with $ \gamma (0) = p $ and $\gamma (1) = q$. Here and henceforth, we will frequently use this $v_q$ notation. 
% This $v_q$ notation will 

When generalizing a smoothing convolution in Euclidean spaces, one's first hunch might be to define an approximation of $f$ (called $\wh{f}^\delta $) such that $ \wh{f}^\delta (p) := \frac{1}{2 \delta A_n} \int_{v \in \S_p} f \( \Exp_p (\delta v)  \) dv $ \citep[e.g., ][]{greene1973subharmonicity}. We want to point out that this $\wh{f}^\delta$ does not make use of the connection between tangent spaces. Instead, our surrogate function is geometry-aware. In particular, it implicitly uses the diffeomorphic property of exponential maps. As we will see, this construction greatly simplified the analysis, and leads to a clean algorithm design. In addition, this local surrogate function gives rise to a global convolution with nice properties, as discussed right below. 

\textbf{A Global Convolution} 

    

With the above surrogate function, we can define a global smoothing of the function $f$, such that 
\begin{align} 
    \widetilde{f}^\delta (p) := \E_{ v \sim \S_p } 
    \[ \widetilde{f}_{p,v}^\delta (p) \] , \label{eq:def-surrogate}
\end{align} 
% Our construction of this surrogate function has several advantages. 
One major advantage is that this function $\wt{f}^\delta$ preserves convexity. We want to remark that, unlike the Euclidean space case, convexity is not preserved after standard convolution ($\wh{f}^\delta$ as discussed above). This is because of the non-trivial curvature on general Riemannian manifolds. In particular, a standard convolution kernel needs strict convexity to ensure convexity only when the convolution width goes to zero \citep[cf. Thereom, 2][]{greene1973subharmonicity}. 

The convexity of $ \wt{f}^\delta (p) $ summarizes to the following Lemma. 

\begin{lemma}
    For a convexity and continuous $f : \M \rightarrow \R$, the function $ \wt{f}^\delta (p) $ (defined in Eq. \ref{eq:def-surrogate}) is convex. 
\end{lemma}

\begin{proof}
    By definition of convexity, we have, for any $p \in \M$, $v \in T_p \M$, and real numbers $\lambda$ and $t$~\footnote{For more general Riemannian manifolds, we can restrict our attention to small $\lambda$ and $t$ so that the exponential map is locally diffeomorphic and the argument is still valid.}, 
\begin{align} 
    f (\Exp_p ((\lambda + t) v )) \hspace{-2pt} + \hspace{-2pt} f (\Exp_p ((-\lambda + t) v )) \hspace{-2pt} \ge \hspace{-2pt} 2 f (\Exp_p (t v )). \label{eq:helper0}
\end{align} 

Let $\gamma (s) = \Exp_p (sv)$ ($s \in [-\lambda-t, \lambda+ t]$) for simplicity. We can thus rewrite (\ref{eq:helper0}) as
\begin{align}
    f ( \Exp_{ \gamma ( \lambda ) } ( t \P_{0,\lambda}^\gamma (v) ) )  +  f ( \Exp_{ \gamma ( -\lambda ) } ( t \P_{0,-\lambda}^\gamma (v) ) )  \ge& 2 f (\Exp_p (t v )) \label{eq:helper1}
\end{align}
Note that $v$ is a tangent vector in $ T_p \M $. 
We can integrate the first term in (\ref{eq:helper1}) with respect to $v$ and $ t $, and get
% can be written as
\begin{align}
    \int_{ v \in \S_p } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( \lambda ) } ( t \P_{0,\lambda}^\gamma (v) ) ) dt \, dv
    =& \int_{ v \in \S_{\gamma(\lambda)}  } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( \lambda ) } ( t v ) ) dt \, dv, \label{eq:helper2}
\end{align}
where we use that parallel transport along geodesics preserves length, for the change of tangent space for the outer integral. 

Now, the term in (\ref{eq:helper2}) is the exact definition of $\wt{f}^\delta (\gamma (\lambda))$. We repeat this computation for the second term in (\ref{eq:helper1}), and get 
\begin{align}
    \wt{f}^\delta (\gamma(\lambda) ) + \wt{f}^\delta (\gamma(-\lambda)) &\ge 2 \wt{f}^\delta (\gamma(0)), 
\end{align}
which is the midpoint convexity (around $ \gamma (0) $) for $\wt{f}^\delta$. 

Since $f$ is continuous, so is $\wt{f}^\delta$. By continuity and midpoint convexity of $\wt{f}^\delta$, we know $\wt{f}^\delta$ is convex. 
\end{proof} 

% We have shown that the surrogate function is convex and a good approximation of the true function. 
Now with the local surrogate function defined, we can move on to the gradient estimation. 
% , and perform gradient descent on this surrogate function.  




\subsection{Single-point Gradient Estimate on Riemannian Manifolds}  

A general recipe to link zeroth order information to first order information is through Stokes' Theorem. However, directly applying Stokes' theorem on Riemannian manifolds requires working with high order differential forms, which can be computationally intense. 
Instead, we use a simple and clean regime: we work with a geodesic curve, and ``rotate'' the curve to recover local geometry of the space. 
In fact, using curves (or low-dimensional surfaces) to describe and/or investigate local properties is one general tool to handle computations and analysis on Riemannian manifolds. 

To start with, we state the following Lemma, as a corollary of the fundamental theorem of calculus. 

% \begin{lemma}
%     \label{lem:fundamental-calculus}
%     Pick $p \in \M$ and $v \in T_p \M$ with $g(v,v)=1$. Let $\Exp_p (t v)$ $(t \in [a,b])$ be a geodesic in $\M$, and let $\gamma (t) = \Exp_p (tv)$ for simplicity. 
%     We then have 
%     \begin{align} 
%         \int_a^b \< \nabla f \big|_{\Exp_p (sv )}, \dot{\gamma}\big|_{s} \> ds = f ( \gamma (b) ) - f ( \gamma (a) ). 
%     \end{align} 
% \end{lemma} 

% \begin{proof}
    
%     Consider the function $f \circ \gamma : [a, b] \rightarrow \mathbb{R}$. By fundamental theorem of calculus, we have 
%     \begin{align*} 
%         f ( \gamma (b) ) - f ( \gamma (a) ) 
%         &= \int_a^b \frac{d f \circ \gamma}{ dt } {d}t . 
%     \end{align*}
%     Also by definition of gradient, 
%     \begin{align*}
%         \frac{d f \circ \gamma}{ dt } \Bigg|_{s} = \lim_{\tau \rightarrow 0} \frac{ f \circ \gamma (s + \tau ) }{ \tau } = \< \nabla f \big|_{\Exp_p (sv )}, \dot{\gamma}\big|_{s} \> . 
%     \end{align*} 
% \end{proof}  



Next, we proceed to prove the following lemma, which provides an estimation scheme for gradient of $f$. 

% \begin{lemma}
%     \label{lem:grad-error}
%     Let $f$ be $\mu$-geodesically smooth. We have 
%     \begin{align}
%         \left\| \nabla f\big|_p - \frac{n}{\delta} \E_{ v \sim \S_p } \[ f \( \Exp_p (\delta v) \) v \] \right\|_p \le \frac{ n \mu \delta }{2}. 
%     \end{align}
% \end{lemma}
% % the constants in (19) are not consistent with (32), please check. 
% % \subsection{Gradient estimate} 

% This lemma provides a very simple gradient estimation scheme: at any point $p$, we can (uniformly) sample a vector $v \in T_p \M$, and $f \( \Exp_p (\delta v) \) v$ gives an estimator of $\nabla f\big|_p$ (up to rescaling). 


% % Let $A_n$ be the surface area of $n$-dimensional unit sphere. 

% % Now, by the above lemma and proposition, and smoothness of function and manifold, we have, 
% % \begin{align}
% %     \nabla \widetilde{f}^\delta \big|_p
% %     &= 
% %     \frac{1}{ A_n } \nabla \int_{v \in \S_p^n }  \widetilde{f}_v^\delta dv = 
% %     \frac{1}{ A_n } \int_{v \in \S_n } \nabla  \widetilde{f}_v^\delta dv = \E_{v \sim \S_n } \[ \nabla \widetilde{f}_v^\delta \] . 
% %     % &= 
% % \end{align} 


% % For a fixed $v\in T_p\M$, $h^\delta(q)= \frac{1}{2\delta}\int_{-\delta}^\delta f(\Exp_q(tv_q)) dt$, where $v_q = P_{\gamma} v$, $\gamma:p\to q$ is the unique geodesic connecting $p$ and $q$. $h$ is defined on a local neighborhood of $p$. 

% % Claim:
% % Firstly, in a neighborhood around $p$, we have 
% % \begin{align}
% %     \nabla \widetilde{f}^\delta 
% %     &= \frac{1}{ A_n } \nabla \int_{v \in \S_p }  f_{p,v}^\delta dv \\ 
% %     & = \frac{1}{ A_n } \int_{v \in \S_p }  \nabla f_{p,v}^\delta dv= \E_{ v \sim \S_p }  \[\nabla f_{p,v}^\delta\], \label{eq:change-grad-int}
% %     % &= 
% % \end{align} 
% % where the exchange of interval and gradient follows from dominated convergence theorem. 
% % \textcolor{red}{We can always exchange the integral and the gradient by imposing extra assumption. What's the best way? }
% \begin{proof}[Proof of Lemma \ref{lem:grad-error}]

% From the definition of directional derivative, we have 
% \begin{align} 
%     &\< \nabla {f}_{p,v}^\delta \big|_p , v \>_p \nonumber \\
%     &\hspace{-10pt}=  \hspace{-2pt} \frac{1}{2\delta} \lim_{ \tau \rightarrow 0 } \hspace{-2pt} \frac{ \int_{-\delta}^\delta \hspace{-2pt} \( \hspace{-2pt} f \hspace{-2pt} \( \Exp_{ \Exp_p (\tau v ) } \hspace{-2pt} \( t v_{\Exp_p (\tau v)} \) \hspace{-2pt} \) \hspace{-2pt} - \hspace{-2pt} f \( \Exp_{p } \hspace{-2pt} \( t v \) \) \hspace{-2pt} \) \hspace{-2pt} dt }{ \tau } \nonumber \\ 
%     &\hspace{-10pt}= 
%   \frac{1}{2\delta} \int_{-\delta}^\delta \lim_{ \tau \rightarrow 0 } \frac{ f \( \Exp_p  \( \tau v + t v \) \) - f \( \Exp_{ p } \( t v \) \)  }{ \tau }  dt \nonumber \\ 
%     &\hspace{-10pt}= \frac{1}{2\delta} \int_{- \delta}^\delta \< \nabla f \big|_{ \Exp_p \( t v \)  } , v_{\Exp_p (tv)} \>_{\Exp_p (tv)} dt  \label{eq:above}
% \end{align} 

% Let $\gamma (t) = \Exp_p (t v)$ ($t \in [-\delta, \delta]$) for notational simplicity. Since $f$ is $\mu$-geodesically smooth, we have, for any $p$ and $v \in T_p \M$,  
% \begin{align}
%     &\< \nabla {f} \big|_p - \nabla {f}_{p,v}^\delta \big|_p , v \>_p \nonumber \\
%     =& 
%     \hspace{-2pt}\< \hspace{-1pt} \nabla {f} \big|_p , v \hspace{-2pt} \>_p \hspace{-2pt}- \hspace{-2pt} \frac{ \int_{- \delta}^\delta \< \nabla f \big|_{ \Exp_p \( t v \)  } , v_{\Exp_p (tv)} \>_{\Exp_p (tv)} dt }{2 \delta} \label{eq:use-above} \\
%     =& 
%     \frac{1}{2 \delta}\int_{- \delta}^\delta \( \< \P_{0,t}^\gamma \( \nabla {f} \big|_p\) , v_{\Exp_p (tv)} \>_{\Exp_p (tv)} \) dt -  \frac{1}{2 \delta}\int_{- \delta}^\delta \( \< \nabla f \big|_{ \Exp_p \( t v \)  } , v_{\Exp_p (tv)} \>_{\Exp_p (tv)} \) dt \label{eq:preserve} \\
%     =& 
%     \frac{1}{2 \delta} \int_{- \delta}^\delta \( \< \P_{0,t}^\gamma \( \nabla {f} \big|_p\) - \nabla f \big|_{ \Exp_p \( t v \)  }, v_{\Exp_p (tv)} \>_{ \Exp_{p} (tv) } \) dt \nonumber \\ 
%     \le& 
%     \frac{1}{2 \delta} \int_{- \delta}^\delta \mu t dt = \frac{\mu \delta}{2} \label{eq:lip}, 
% \end{align} 
% where (\ref{eq:use-above}) uses (\ref{eq:above}), and (\ref{eq:preserve}) uses the fact that the parallel transport preserves the Riemannian metric. 


% By Proposition \ref{prop:inner-prod}, we have 
% \begin{align*}
%     \E_{v \in \S_p} \[ \< \nabla f \big|_p, v \>_p v \] = \frac{1}{n} \nabla f \big|_p,
% \end{align*}  
% and thus from (\ref{eq:lip}), we have 
% \begin{align}
%     \left\| \E_{v \in \S_p} \[ \< \nabla f_{p,v}^\delta \big|_p, v \>_p v \] - \frac{1}{n} \nabla f \big|_p \right\|_p \le \frac{ \mu \delta}{2}. \label{eq:est-error} 
% \end{align}

% % Together with (\ref{eq:change-grad-int}) and (27), this gives
% % \begin{align} 
% %     holder
% % \end{align} 

% % Now we move back to . 
% Applying the Lemma \ref{lem:fundamental-calculus} and the above results gives 
% \begin{align}
%     % &\nabla \widetilde{f}^\delta \big|_p \nonumber \\
%     % =& 
%     % \frac{n}{2} 
%     &\E_{v \sim \S_p } \[ \< \nabla {f}_{p,v}^\delta \big|_p , v \>_p v \] \nonumber \\
%     =&  
%     % \frac{n}{2} 
%     \E_{v \sim \S_p } \[ \frac{1}{2 \delta} \int_{- \delta}^\delta \< \nabla f \big|_{ \Exp_p \( t v \) } , v_{\Exp_v} \>_{\Exp_p (v)}  dt \; v \] \tag{by Eq. \ref{eq:above}} \\
%     =& 
%     % \frac{n}{2} 
%     \frac{1}{2 \delta} \E_{v \sim \S_p } \[ \( f \( \Exp_p (\delta v) \) - f \( \Exp_p (\delta v) \) \)  v \] \tag{by Lemma \ref{lem:fundamental-calculus}}\\ 
%     =& 
%     \frac{1}{\delta} \E_{ v \sim \S_p } \[ f \( \Exp_p (\delta v) \) v \] . \nonumber
% \end{align}

% Combining the above result with (\ref{eq:est-error}) gives
% \begin{align}
%     \left\| \nabla f\big|_p - \frac{n}{\delta} \E_{ v \sim \S_p } \[ f \( \Exp_p (\delta v) \) v \] \right\|_p \le \frac{n \mu \delta}{2}. 
% \end{align}

% \end{proof}



% The above derivation gives a fairly convenient gradient approximation scheme: 

% At any point $p$, sample a vector $v \sim \S_p$, travel to the point $ \Exp_p ( \delta v ) $, and observe the function value $ f \( \Exp_p (\delta v) \) $. Then  $ f \( \Exp_p (\delta v) \) v $ gives an estimate for $ \nabla \widetilde{f}^\delta \big|_p $, as


% \subsection{Convexity of the surrogate function}

% For a geodesic $ \gamma: [a,b] \rightarrow \M $, and $v \in T_{\gamma (c)} \M$ ($c \in [a,b]$), we use $ \P_{c , d }^\gamma (v) $ ($d \in [a,b]$) to denote the parallel transport of $v$ from $\gamma (c)$ to $\gamma (d)$.  

% By definition of convexity, we have, for any $p$ and small $\lambda$ and $t$, 
% \begin{align} 
%     f (\Exp_p ((\lambda + t) v )) + f (\Exp_p ((-\lambda + t) v )) \ge 2 f (\Exp_p (t v )). 
% \end{align} 

% Let $\gamma (s) = \Exp_p (sv)$ ($s \in [-\lambda-t, \lambda+ t]$) for simplicity. We thus have,
% \begin{align}
%     f ( \Exp_{ \gamma ( \lambda ) } ( t \P_{0,\lambda}^\gamma (v) ) )  +  f ( \Exp_{ \gamma ( -\lambda ) } ( t \P_{0,-\lambda}^\gamma (v) ) ) &\ge 2 f (\Exp_p (t v )) \\
%     \int_{ v \in T_p \M } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( \lambda ) } ( t \P_{0,\lambda}^\gamma (v) ) ) dt \, dv + \int_{ v \in T_p \M } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( -\lambda ) } ( t \P_{0,-\lambda}^\gamma (v) ) ) dt \, dv &\ge 2 \int_{ v \in T_p \M } \int_{-\delta}^\delta f (\Exp_p (t v )) dt \, dv \\ 
%     \int_{ v \in T_{\gamma(\lambda)} \M } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( \lambda ) } ( t v ) ) dt \, dv + \int_{ v \in T_{\gamma (-\lambda)} \M } \int_{-\delta}^\delta f ( \Exp_{ \gamma ( -\lambda ) } ( t v ) ) dt \, dv &\ge 2 \int_{ v \in T_p \M } \int_{-\delta}^\delta f (\Exp_p (t v )) dt \, dv  \\ 
%     \wt{f}^\delta (\gamma(\lambda) ) + \wt{f}^\delta (\gamma(-\lambda)) &\ge 2 \wt{f}^\delta (\gamma(0)). 
% \end{align}
% The continuity and midpoint convexity of $\wt{f}^\delta $ implies its convexity. 


% \subsection{Convexity of Inscribed Set}

% For a geodesically convex set compact $\D \subseteq \M$ and $\alpha > 0$, we use $ (1 - \alpha) \D $ to denote the set such that 
% \begin{align}
%     &(1 - \alpha ) \D := \Bigg\{ p \in \D: 
%     \Exp_p (\alpha v) \in \D, \, \forall v \in \S_p, \nonumber
%     \\
%     &\quad \text{and } \exists v \in \S_p, s.t., \Exp_{p} ((\alpha + \epsilon ) v) \notin \D, \, \forall \epsilon > 0 \Bigg\}. 
% \end{align}

% With the above gradient estimator, we are now 
\subsection{Gradient descent with biased gradient estimator} 

With the above gradient estimator and projection on to $(1 - \alpha) \D$ defined, we can now perform gradient-type analysis. To start with, we quote the following Lemma. 

\begin{lemma}[Corollary 8, \citet{zhang2016first}] 
    \label{lem:zhang}
    Let $\M$ be a Riemannian manifold, 
    % For any $p \in \M $ and $u,v \in T_p \M$, i
    with sectional curvature $ \mathcal{K}_p (u,v) \ge \kappa > -\infty$ for all $p \in \M$ and $u,v \in T_p \M$. Then for any $x, x_s$, and $x_{s+1} = \Exp_{x_s} (-\eta v)$ for some $v \in T_{x_s} \M$, it holds that 
    \begin{align}
        \< - v , \Exp_{x_s}^{-1} (x) \>_{x_s} \le& \frac{1}{2 \eta } \( d^2 (x_s, x) - d^2 (x_{s+1}, x) \) + \frac{\zeta (\kappa, d(x_s, x)) \eta }{2} \| v \|^2, \nonumber
    \end{align}
    where $ \zeta (\kappa, D) = \frac{ \sqrt{|\kappa|} D }{ \tanh (\sqrt{|\kappa|} D ) } $. 
\end{lemma}
% \subsection{Quadratic Bound for Geodesically Smooth Functions}


% \begin{align}
%     f (y) \le f (x) + \< \nabla f\big|_x , \Exp_x^{-1} (y) \>_x + \frac{\mu}{2}  d (y,x). 
% \end{align} 
% Let $x \leftarrow x_{t}$ and $y \leftarrow \Exp_{x_t} ( -\eta w_t )$, we have 
% \begin{align}
%     f (x_{t+1}) 
%     &\le f (x_t) + \< \nabla f\big|_{x_t} , \Exp_{x_t}^{-1} (x_{t+1}) \>_{x_t} + \frac{\mu}{2}  d^2 (x_{t+1},x_t) \\
%     &= 
%     f (x_t) + \< \nabla f\big|_{x_t} , \Exp_{x_t}^{-1} (x_{t+1}) \>_{x_t} + \frac{\mu}{2}  \eta^2 \| w_t \|_{x_t}^2 \\
%     &\le 
%     f (x_t) + \< \nabla f\big|_{x_t} , -\eta w_t \>_{x_t} + \frac{\mu}{2}  \eta^2 \| w_t \|_{x_t}^2. 
% \end{align} 

% Recall $w_t = $
% In expectation,
% \begin{align}
%     \E \[ f (x_{t+1}) \]
%     &\le 
%     \E \[ f (x_t) \] + \E \[ \< \nabla f\big|_{x_t} , -\eta w_t \>_{x_t} \] + 
%     \E \[ \frac{\mu}{2}  \eta^2 \| w_t \|_{x_t}^2 \] \\
%     &\le 
%     % \E \[ f (x_t) \] - \| \E \[ w_t\] \| \(  \| \E \[ w_t \] \| - n\mu\delta  \) + \E \[ \frac{\mu}{2}  \eta^2 \| w_t \|_{x_t}^2 \] 
%     % &\le 
% \end{align} 

% By convexity, we have 
% \begin{align}
%     f (x) \le f (x^*) + 
% \end{align}



% When $\alpha \ge \delta$, our local surrogate function is locally defined around any point $p \in (1 - \alpha) \D$. 

% \textcolor{red}{We then perform gradient descent to minimize the surrogate function. Then the surrogate function approximate the true function, our algorithm will find an approximate optimum of the function. }

%Let's use $K_p (u,v)$ to denote the sectional curvature of the the sub-manifold of $\M$ spanned by $u,v \in T_p \M $.
% The following theorem gives a bound for gradient descent type algorithms. 


% We need to show that the surrogate function is convex. 

Gathering all above analysis proves Theorem \ref{thm:rate} 

\begin{proof}[Proof of Theorem \ref{thm:rate}]
    % Firstly, 
    % \begin{align}
    %     d \(x_{t+\frac{1}{2}} , x_{t+ 1} \) \le \alpha, \quad  \forall t. 
    % \end{align} 
    By convexity of $f$, we have $ f(x_{t + 1}) - f(x^*) \le  \< - \nabla f\big|_{x_{t+1} }, \Exp_{ x_{t+1} }^{-1} (x^*) \> $. 
    % Together 
    Together with the Lemma of Zhang and Sra, we get
    \begin{align*}
        % &f ( x_t ) - f (x^*)  \\
        % \le&
        &f ( x_{t } ) - f (x^*) \\
        \le& \< - \nabla f\big|_{x_{t} }, \Exp_{x_{t } }^{-1} (x^*) \> \\
        \le& \< - w_t, \Exp_{x_{t } }^{-1} (x^*) \> + \< w_t - \nabla f\big|_{x_{t} }, \Exp_{x_{t } }^{-1} (x^*) \> \\
        % + f ( x_{t + 1 } )  
        % - f ( x_{t + \frac{1}{2}} ) \\
        \le& 
        \frac{1}{2 \eta } 
        \( d^2 (x_{t}, x^*) - d^2 
        (x_{t+\frac{1}{2}}, x^*) \) + 
        \frac{\zeta (\kappa, D) \eta }{2} \| w_t \|^2 + \< w_t - \nabla f\big|_{x_{t} }, \Exp_{x_{t } }^{-1} (x^*) \>,
    \end{align*}
    where the last line uses Lemma \ref{lem:zhang}. Taking expectation (over $v_t \sim \S_{x_t}$) on both sides gives 
    \begin{align}
        &\E \[ f ( x_{t } ) \] - \E \[ f (x^*) \] \nonumber \\
        \le& 
        \frac{1}{2 \eta } 
        \E \[ d^2 (x_{t}, x^*) - d^2 
        (x_{t+\frac{1}{2}}, x^*) \] \hspace{-2pt} + \hspace{-2pt}
        \E \[ \frac{\zeta (\kappa, D) \eta }{2} \| w_t \|^2 \] + \< \E \[ w_t\] - \nabla f\big|_{x_{t} }, \Exp_{x_{t } }^{-1} (x^*) \> \nonumber \\
        \le& 
        % \frac{1}{2 \eta } 
        \frac{ \E \hspace{-2pt} \[ d^2 ( \hspace{-1pt} x_{t}, \hspace{-1pt} x^* \hspace{-1pt} )  \hspace{-2pt} - \hspace{-2pt} d^2 ( \hspace{-1pt} x_{t+\frac{1}{2}}, \hspace{-1pt} x^* \hspace{-1pt} ) \hspace{-1.5pt} \] }{ 2 \eta } \hspace{-2pt} + \hspace{-3pt} \frac{D \mu \delta }{2} + \hspace{-2pt}
        \frac{\zeta (\kappa,\hspace{-2pt} D) \eta n^2 G^2 }{2 \delta^2  } \hspace{-3pt}, \label{eq:anchor} 
    \end{align} 
    where the last line uses Lemma \ref{lem:grad-error}, and that $ \|w_t \|^2 \le \frac{n^2 G^2 }{ \delta^2 } $ ($G \ge f (p) $ for all $p \in \D$). 
    Note that the above argument is true only in expectation. Henceforth, we will omit the expectation operator $\E$ for simplicity. 
    
    % Let $ $. 
    By definition of $ (1 - \delta) \D $, we have, $ d \(x_{t+\frac{1}{2}} , x_{t+ 1} \) \le \delta $. Lipschitzness of function $f$ gives $ \left| f \(x_{t+\frac{1}{2}} \)- f \( x_{t+ 1} \) \right |\le \delta L $. Plugging this back to (\ref{eq:anchor}), we get, in expectation, 
    \begin{align*}
        &f ( x_t ) - f (x^*) \le
        \frac{1}{2 \eta } 
        \( d^2 (x_{t}, x^*) - d^2 
        (x_{t+1}, x^*) \) + 
        \frac{\zeta (\kappa,\hspace{-2pt} D) \eta n^2 G^2 }{2 \delta^2  } + \( L + \frac{D\mu n}{2} \) \delta . 
    \end{align*} 
    %     d \(x_{t+\frac{1}{2}} , x_{t+ 1} \) \le \alpha, \quad  \forall t. 
    % \end{align} $
    
    % Let $G = \sup_{p \in \D} f ( p )$. 
    % Since $w_t = \frac{n}{\delta} f \( \Exp_p \( \delta v_t \) \) v_t$, we have
    Summing over $t$ gives, in expectation, 
    \begin{align*}
        &\sum_{t=1}^T f ( x_t ) - f (x^*) \\
        \le& \frac{1}{2 \eta }
        \sum_{t=1}^T \( d^2 (x_{t}, x^*) - d^2 (x_{t+1}, x^*)  \) +
        \frac{\zeta (\kappa, D) \eta n^2 G^2 T }{2\delta^2 } + \( L + \frac{D\mu n}{2} \) \delta T \\
        \le& 
        \frac{D^2}{2\eta} + \frac{\zeta (\kappa, D) \eta n^2 G^2 T }{2\delta^2 }  + \( L + \frac{D\mu n}{2} \) \delta T, 
    \end{align*}
    where the last line telescopes out the summation term. 
    % which gives
    % \begin{align}
    %     \frac{1}{T} \sum_{t=1}^T f ( x_t ) - f (x^*) \le \frac{D}{2\eta T} + D \alpha + \frac{\zeta (\kappa, d(x_t, x^*)) \eta n^2 G^2 }{2\delta^2}.
    % \end{align}
    By convexity of $f$, 
    \begin{align*}
        f ( \bar{x}_T ) \le \frac{1}{T} \sum_{t=1}^T f ( x_t ), 
    \end{align*}
    which concludes the proof. 
    
\end{proof} 

\begin{figure*}[t]
    \centering
    \includegraphics[scale = 0.5]{figures/A10Seta0.005delta0.1.png} \includegraphics[scale = 0.5]{figures/A100Seta0.005delta0.1.png}
    \caption{This figure shows the performance of {Alg}orithm \ref{alg} with {S}tabilized gradient estimators (thus labelled Alg1-S). Both solid lines are average performance of 5 runs. The width of shaded area above and below the solid line represents $ps$ one standard deviation. In both plots, $\eta = 0.005$ and $\delta = 0.1$. In the left sub-figure, 10 random  positive definite matrices $A_i$ are randomly sampled. In the right sub-figure, 100 random  positive definite matrices $A_i$ are randomly sampled. \label{fig} }
\end{figure*}


==> tex/background.tex <==
\section{Background}

\subsection*{Riemannian Geometry} 

A Riemannian manifold $ (\M, g) $ is a smooth manifold equipped with a metric tensor $g$ such that at any point $p \in \M$, $g_p$ defines a positive definite inner product in the tangent space $T_p\M$. For a point $p \in \M$, we use $ \< , \>_p $ to denote the inner product in $T_p \M$ induced by $g$. Also, we use $\|\cdot \|_p $ to denote the norm associated with $ \< ,\>_p $. Intuitively, a Riemannian manifold is a space that can be locally identified as an Euclidean space. With such structures, one can locally carry out calculus and linear algebra operations.  

A vector field $X$ assigns each point $p \in \M$ a unique vector in $T_p \M$. Let $\mathfrak{X}(\M)$ be the space of all smooth vector fields. An affine connection is a mapping 
% a second order derivative on manifold $\M$, denoted by, 
$\nabla: \mathfrak{X}(\M)\times \mathfrak{X}(\M) \rightarrow \mathfrak{X}(\M)$  so that (i) $ \nabla_{f_1 X_1 + f_2 X_2 } Y = f \nabla_{X_1} Y  + f_2 \nabla_{ X_2 } Y$ for $f_1, f_2 \in C^\infty (\M)$, (ii) $ \nabla_{X } (a_1 Y_1 + a_2 Y_2) = a_1 \nabla_{X} Y_1 + a_2 \nabla_X Y_2$ for $a_1, a_2 \in \R $, and (iii) $ \nabla_{X } (f Y) = f \nabla_{X } Y + X(f) Y $ for all $f \in C^\infty (\M)$. The  Riemannian connection, also known as the Levi-Civita connection, is the unique torsion free affine connection that 
% is torsion-free~\footnote{For the purpose of our paper, it is not necessary to understand.} and 
is compatible with the Riemannian metric $g$. %, which we will explain as we define parallel transport%~\footnote{A Riemannian metric is also torsion-free, but we omit the discussion on this property for the purpose of this paper. }. 
A geodesic curve $\gamma: [0,1] \rightarrow \M$ is a curve so that $\nabla_{\dot{\gamma}(t)} \dot{\gamma}(t) = 0$ for all $t \in [0,1]$, where $ \nabla $ here denotes the Riemannian connection. Intuitively, this means there is no acceleration along the curve. One can think of geodesic curves as generalizations of straight line segments in Euclidean space. At any point $p \in \M$, the exponential map $\Exp_p$ is a local diffeomorphism that maps $v \in T_p\M$ to $\Exp_p (v) \in \M$ such that there exists a geodesic curve $\gamma : [0,1] \rightarrow \M$ with $ \gamma (0) = p $, $ \dot{\gamma}\big|_0 = v $ and $\gamma(1)=\Exp_p (v)$. Since the exponential map is (locally) diffeomorphic, the inverse exponential map is also properly defined (locally). We use $\Exp_p^{-1}$ to denote the inverse exponential map of $\Exp_p$. 

% With geodesic curve defined, 

We say a vector field $X$ is parallel along a geodesic $\gamma: [0,1] \rightarrow \M$ if 
$ \nabla_{\dot{\gamma} (t)} X = 0 $ for all $t\in[0,1]$. For $t_0, t_1 \in [0,1]$, we call the map $ \P_{t_0, t_1}^{\gamma} : T_{\gamma (t_0)} \M \rightarrow T_{\gamma (t_1)} \M $ a parallel transport, if it holds that for any vector field $X$ such that $X$ is parallel along $\gamma$, $X (\gamma (t_0)) $ is mapped to $X (\gamma (t_1)) $. Parallel transport induced by a Riemannian connection preserves the Riemannian metric, that is, for $p\in \M$, $u,v \in T_p \M$, and geodesic $\gamma : [0,1] \rightarrow \M$, it holds that $\< u,v \>_{\gamma(0)} = \< \P_{0,t}^\gamma (u), \P_{0,t}^\gamma (v) \>_{\gamma(t)}$ for any $t \in [0,1]$. 

The curvature tensor $\mathcal{R}:\mathfrak{X}(\M)\times\mathfrak{X}(\M)\times \mathfrak{X}(\M)\to\mathfrak{X}(\M)$ is defined as $\mathcal{R}(X,Y)Z = \nabla_X\nabla_YZ-\nabla_Y\nabla_X Z-\nabla_{[X,Y]}Z$, where $[,]$ is the Poission bracket on $\M$.  The sectional curvature $\mathcal{K}:\mathfrak{X}(\M)\times\mathfrak{X}(\M)\to\mathbb{R}$ is defined as $\mathcal{K}(X,Y)=\frac{g(\mathcal{R}(X,Y)X,Y)}{g(X,X)g(Y,Y)-g(X,Y)^2}$, which is the high dimensional generalization of Gaussian curvature. Intuitively, for a point $p$, $\mathcal{K} \( X(p), Y (p) \)$ is the the Gaussian curvature of the sub-manifold spanned by $  X(p), Y(p)$ at $p$. For all $ p \in \M $ and $u,v \in T_p \M$, we write $ \mathcal{K}_p (u,v) := \mathcal{K} \( X(p), Y (p) \) $ for some $X$ and $Y$ such that $X(p) = u$ and $Y(p) = v$. If a complete, simply connected Riemannian manifold has no where positive sectional curvature, the exponential map $\Exp$ is a global diffeomorphism \citep[Cartan-Hadamard theorem,][]{kobayashi1963foundations} and the manifold is called a Hadamard manifold. 

==> tex/lower-bound.tex <==
\section{Lower Bound} 

We call an ordering of a Cartesian coordinate of Euclidean space an \textbf{orientation}/\textbf{handedness}. Fix an orientation $\H$ of the Euclidean coordinate for $\R^{n\times n}$. With respect to $\H$, for $v \in \R^{n\times n}$, let $v_i $ be the $i$-th (out of $n \times n$) coordinate of $v$. With respect to $\H$, we define a partial order $ \succeq_{\H}  $ in $\R^{n \times n}$, such that $v \succeq_{\H} v'$ if either (1) $v = v'$ or (2) $ v_{i^*} > v_{i^*}' $ where $i^* = \min \{ i : v_{i} \neq v_i' \}$. 


Construct the following parametrization of points in $GL_n(\R)$. 
Given an orientation $\H$, for any point $x \in GL_n(\R)$, fine the tangent vectors $v_x$ at $I$ such that $v_{x, \H } = \arg \min_{v, \H } \{ v: \exp (v) = x \}$, where the minimum is taken with respect to the partial ordering $ \succeq_{\H}$. 
% If there are two tangent vectors $v_x$ and $v_x'$ such that $ \exp (v_x) = \exp \( v_x' \) $, we pick $  $. With respect to the coordinate ordering (of the Euclidean space) $\R^{n \times n}$, $v_x ( )$. we  
The coordinate of $x$ (with respect to $\H$) is defined to be the coordinate of $v_{x, \H}$. Due to the non-commutative nature of the space $GL_n \(\R \)$, this coordinate system is ``intrinsically different'' from another such coordinate system with a different orientation. For easier reference, we call such coordinate system $ \Co_{\H} $. 

With coordinate system $ \Co_{\H} $, for a vector $ e \in \R^{n\times n} $, define function $f_e: GL_n (\R) \rightarrow \R $ such that 
\begin{align}
    f_e (x) = \( d (x, I) \)^2 + \sum_{i=1}^{n^2} \frac{ e_i x_{i, \H } }{ 1 + \( x_{i, \H} / e_i \)^2 }. 
\end{align} 

\subsection{Properties of the function $f_e$. Most importantly convexity (and smoothness). }

Recall from above the definition of strong convexity. 
At any $x, y \in GL_n \( \R \)$
\begin{align} 
    f_e (x ) - f_e (y) 
\end{align} 


==> tex/maybe-useful.tex <==

\begin{definition}[Radial Hessian]
\label{def:rad-hess}
Consider a point $p \in \M$, a local coordinate for $T_p \M$ and a fixed positive number $\sigma^2$. For $f \in C^{\infty} (\M)$ and $p \in \M$ define the radial Hessian of $f$ at $p$ as $ H_{f,p} : T_p \M  \times T_p \M \rightarrow \R$ such that 
% \begin{align*} 
%     H_{p, f} := \E_u \[ u u^\top  \lim_{\tau_1 \rightarrow 0} \lim_{\tau_2 \rightarrow 0} \frac{ f ( \Exp_p ( \(\tau_1 + \tau_2\) u / \| u \| ) ) - f ( \Exp_p ( \(\tau_1 -\tau_2\) u / \| u \| ) ) - f ( \Exp_p ( \(-\tau_1 +\tau_2\) u / \| u \| ) ) + f ( \Exp_p ( \(-\tau_1 -\tau_2\) u / \| u \| ) ) }{4\tau_1 \tau_2}  \]. 
% \end{align*} 
\begin{align*} 
    H_{p, f} := \frac{1}{ 2 \sigma^4 } \E \[ \( u u^\top - I \) D_{uu} f (p) \], 
\end{align*} 
where 1. $u = [u_1, u_2, \cdots, u_n]^\top $ with $u_i \overset{i.i.d.}{\sim} \mathcal{N} (0, \sigma^2)$, and 2. 
\begin{align}
    D_{uu} f (p) =  \lim_{\tau \rightarrow 0}  \frac{ f ( \Exp_p ( \tau u  ) ) - 2 f ( p ) + f ( \Exp_p ( - \tau u  ) ) }{\tau^2} . 
\end{align}
\end{definition} 

The radial Hessian generalizes the Hessian matrix in Euclidean spaces and agrees with the Hessian in Definition \ref{def:hessian} locally. Also, one can use the radial Hessian for second order convexity test and allows easier computation of the Hessian. These facts can be found in Propositions \ref{prop:rad-hess-gen} and \ref{prop:sec-order}. 



% For any $p \in \M$, with the normal coordinate specified by the exponential map $\Exp_p$, the Christoffel symbol vanishes at $p$. This means that 
% We introduce the 

\begin{proposition}
    \label{prop:rad-hess-gen}
    For the Euclidean space $ \R^n $ and a function $f \in C^{\infty} (\R^n)$, it holds that 
    \begin{align} 
        \( H_{p,f} \)_{kh} = \partial_k \partial_h f \big|_p, \quad \forall p \in \R^n. 
    \end{align} 
\end{proposition} 

\begin{proof} 
    % For a vector $u$, let $u_0 = u / \| u \|$. 
    Since $D_{uu} f(p) = u^{i} u^{j} \partial_i \partial_j f \big|_p$ for all $u \in T_p \M$, it suffices to consider
    % \begin{align*}
    $  u_k u_h  u_{i} u_{j} \partial_i \partial_j . $ 
    % \end{align*} 
    
    When $(k,h) = (i,j)$, one has $ \E \[ u_k u_h u_i u_j \partial_i \partial_j \] = \E \[ u_i^2 u_j^2 \partial_i \partial_j \] $. In this case, it holds that 
    \begin{align*} 
        \E \[ u_i^2 u_j^2 \partial_i \partial_j \] 
        &= \sigma^4 \partial_k \partial_h \quad \text{for } i \neq j \quad \text{and} \quad \E \[ u_i^4 \partial_i \partial_i \] = 3 \sigma^4 \partial_k \partial_k , \quad \text{for } i = j. 
    \end{align*} 
    
    When $(k,h) \neq (i,j)$, $ i = j$ and $k = h$, we have $ \E \[ u_k^2 u_i^2 \partial_i \partial_j \] = \sigma^4 \partial_i \partial_i $. 
    
    When $(k,h) \neq (i,j)$, $ i = j$ and $k\neq h$, we have $ \E \[ u_k u_h u_i u_j \] = 0 $. 
    
    When $(k,h) \neq (i,j)$, $ i \neq j$ and $k= h$, we have $ \E \[ u_k u_h u_i u_j \] = 0 $.
    
    When $(k,h) \neq (i,j)$, $ i \neq j$, $k\neq h$, $k = j$ and $h=i $, we have $ \E \[ u_k u_h u_i u_j \partial_i \partial_j \] = \E \[ u_i^2 u_j^2 \partial_h \partial_k \] =  \sigma^4 \partial_h \partial_k $. 
    
    When $(k,h) \neq (i,j)$, $ i \neq j$, $k\neq h$, $k = i$ and $h=j $, we have $ \E \[ u_k u_h u_i u_j \partial_i \partial_j \] = \E \[ u_i^2 u_j^2 \partial_k \partial_h \] = \sigma^4 \partial_k \partial_h $. 
    
    When $(k,h) \neq (i,j)$, $ i \neq j$, $k\neq h$ and $k \neq j$, we have $ \E \[ u_k u_h u_i u_j \] = 0 $. 
    
    When $(k,h) \neq (i,j)$, $ i \neq j$, $k\neq h$ and $h \neq i$, we have $ \E \[ u_k u_h u_i u_j \] = 0 $. 
    
    Combining all above cases gives 
    \begin{align} 
        \E \[  u_k u_h  u^i u^j \partial_i \partial_j \] 
        =& 
        \sigma^4 \partial_k \partial_h (1 - \delta_{kh}) + \sigma^4 \partial_h \partial_k (1 - \delta_{hk}) + \delta_{kh} \sum_i \sigma^4 \partial_i \partial_i + 2 \sigma^4 \partial_k \partial_k \nonumber \\
        =& 
        2 \sigma^4 \partial_k \partial_h + \delta_{kh} \sum_i \sigma^4 \partial_i \partial_i . \nonumber
        % \E \[ \delta_{kh} \sum_{ij} u_i u_j  \partial_i \partial_j  \] . 
    \end{align} 
    Since $ \E \[ \delta_{kh} u^i u^j  \partial_i \partial_j  \] =  \delta_{kh} \sum_i \sigma^4 \partial_i \partial_i $, 
    rearranging terms finishes the proof. 
\end{proof} 

\begin{proposition}[Second Order Convexity Test]
    \label{prop:sec-order}
    For a smooth function $f$ defined over a complete Riemannian manifold, it holds that $v^\top H_{p,f} v = D_{vv} f (p)$ for all $v \in T_p \M$. Also, the radial Hessian $H_{p,f}$ is positive semi-definite if and only if $ f $ is convex at $p$. 
\end{proposition}

\begin{proof}
    
    In the proof of Proposition \ref{prop:rad-hess-gen}, we have shown that 
    \begin{align} 
        \E \[ \frac{1}{2\sigma^4} \( u_k u_h - \delta_{kh} \)  u^i u^j \partial_i \partial_j \] = \partial_k \partial_h. 
    \end{align} 
    
    Thus it holds that 
    \begin{align}
        v^\top H_{p,f} v = v^\top \( \frac{1}{ 2 \sigma^4 } \E \[ \( u u^\top - I \) D_{uu} f (p) \] \) v = v^k v^h \partial_k \partial_h f \big|_p = D_{vv} f (p), 
    \end{align} 
    which concludes the proof. 
    
\end{proof} 

==> tex/variance.tex <==

% \section{variance}




